A Novel Model for Vulnerability Analysis through Enhanced Directed Graphs and Quantitative Metrics

Industrial components are of high importance because they control critical infrastructures that form the lifeline of modern societies. However, the rapid evolution of industrial components, together with the new paradigm of Industry 4.0, and the new connectivity features that will be introduced by the 5G technology, all increase the likelihood of security incidents. These incidents are caused by the vulnerabilities present in these devices. In addition, although international standards define tasks to assess vulnerabilities, they do not specify any particular method. Having a secure design is important, but is also complex, costly, and an extra factor to manage during the lifespan of the device. This paper presents a model to analyze the known vulnerabilities of industrial components over time. The proposed model is based on two main elements: a directed graph representation of the internal structure of the component, and a set of quantitative metrics that are based on international security standards; such as, the Common Vulnerability Scoring System (CVSS). This model is applied throughout the entire lifespan of a device to track vulnerabilities, identify new requirements, root causes, and test cases. The proposed model also helps to prioritize patching activities. To test its potential, the proposed model is applied to the OpenPLC project. The results show that most of the root causes of these vulnerabilities are related to memory buffer operations and are concentrated in the \textit{libssl} library. Consequently, new requirements and test cases were generated from the obtained data.

==> docs/6.Biography.tex <==
% =================================================================================
% === IX. BIOGRAPHY ===============================================================
% =================================================================================
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo/angel_BW.jpg}}]{Ángel Longueira-Romero} Ángel Longueira Romero was born in Venezuela in 1994. He received B.S. and M.S. degrees in Industrial Electronics and Automation Engineering from the University of Oviedo in 2017 and 2019, respectively. He is currently working on his Ph.D. degree with the Cybersecurity in embedded Systems Team at Ikerlan Technology Research Center, in Arrasate/Mondragón, Spain.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo/rosa_BW.jpg}}]{Rosa Iglesias} is a senior researcher at the Industrial Cybersecurity Area at IKERLAN, Spain. After graduating in Mathematics, she obtained her Ph.D. in Computer Science at the University of the Basque Country, with stages at MIT (Boston) and University of Belfast (Ireland). She also held a post-doctoral position at SITE, University of Ottawa (Canada). She is certified as CyberSecurity Specialist by TÜV Rheinland. Her current research interests span many aspects of industrial cybersecurity, including standards such as IEC 62443, vulnerability testing, risk analysis and penetration testing. She has wide experience in industrial projects, and national and European research projects. She has published many refereed publications in journals and international conferences. She collaborates as a member of the National Cybersecurity Forum.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo/flores_BW.jpg}}]{Jose Luis Flores} is a researcher at Ikerlan Technology Research Center, is currently part of the Cybersecurity in Embedded System team. He holds a M.Sc. in Robotics and Advanced Control from the University of the Basque Country. His main interest is related to Artificial Intelligence and Cybersecurity. As such, the main lines he works on in each organization are Embedded System security at Ikerlan, Machine Learning and Optimization at the university.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photo/igaritano.png}}]{Iñaki Garitano} is lecturer/researcher at Mondragon Unibertsitatea in the Data Analysis and Cybersecurity research team. Prior to that, he worked as a postdoctoral fellow at UNIK-University Graduate Centre, Norway. He received his Ph.D. from the Department of Electronics and Computer Science, Mondragon Unibertsitatea in 2014 in the area of industrial control systems security. His research interests include security, data science, industrial automation and control systems, and information and communication networks, including the Internet of Things. He currently participates in several European, national and regional level public funding projects.
\end{IEEEbiography}

==> docs/aux.tex <==
% =================================================================================
% === V. DESCRIPTION OF THE PROPOSED MODEL ========================================
% =================================================================================
% \section{A Novel Methodology For Vulnerability Analysis}
    \subsection{Description of the Model}
    \label{sec:modelDescription}
        The model proposed in this research work is based on directed graphs, and requires knowledge of the internal structure of the device to be evaluated, i.e., the assets that comprise it and the relationships between them. Therefore, this section defines the most basic elements that make up the model: system under test, assets, weaknesses, vulnerabilities, and extended dependency graphs.

% ----------------------------------------
% --------- EXTENDED DEPENDENCY GRAPH ----
% ----------------------------------------
            
        \begin{definition}
            A System Under Test (SUT) is now represented by an Extended Dependency Graph (EDG) model $G = \left( \langle A, V \rangle, E \right)$ based on directed graphs, where $A$ and $V$ represents the nodes of the graphs, and $E$, its dependencies. Together with the graph, a set of metrics $M$ is also defined:
            \begin{itemize}
                \item $A = \{a_1, ..., a_n\}$ represents the set of assets in which the SUT can be decomposed, being $n$ the total number of obtained assets. An asset $a$ is any component of the SUT that supports information-related activities and include both hardware and software~\cite{MAGERIT, enisa_glossary, ISO_13335_2004}. 
                Each asset will be characterized with its corresponding CPE identifier, using the existing one whenever is possible, or creating one following the CPE Naming Specification~\cite{CPE7695} when there is no CPE available. Following the denomination in the ISA/IEC 62443 standard~\cite{IEC62443}, the SUT may be an industrial component, a part of an industrial component, a set of industrial components, a unique technology that may never be made into a product, or a combination of these.
                Each asset will also contain information about the weaknesses present that can give rise to vulnerabilities, using their corresponding CWE identifier.
                In the EDG model, assets will be represented by two types of nodes in the directed graphs, \textit{i.e.}, asset nodes and supernodes.
                \item $V = \{v_1, ..., v_q\}$ represents the set of known vulnerabilities that are present in each asset of $A$, being $q$ the total number of vulnerabilities. They are characterized with the corresponding CVE and CVSS values. 
                In the EDG model, vulnerabilities will be represented using two types of nodes in the directed graphs, \textit{i.e.}, known vulnerability nodes and supernodes.
                \item $M = \{m_1, ..., m_r\}$ represents the set of metrics defined in this research work, being $r$ the total number of metrics. This set can be extended, defining more metrics according to the nature of the SUT.
                \item $E = \{e_{ij} | \forall i, j \in \{1, ..., n+q\} \text{ such that } i \neq j \}$ represents the set of relations or dependencies between assets and vulnerabilities. $e_{ij}$ indicates that a dependency relation is established from the asset $a_i$ to the asset $a_j$.
                Dependencies will be represented using two different types of arrows in the EDG, \textit{i.e.}, normal dependency and deprecated asset/updated vulnerability nodes.
            \end{itemize}
        \end{definition}

        In other words, the EDG model can represent a system, from its assets, vulnerabilities, and dependencies as a directed graph. Assets and vulnerabilities are represented as nodes, and their dependencies are represented as arcs in the graph. The information in the EDG is further enhanced, introducing metrics. That said, the EDG model of a given SUT will include four types of nodes and two types of dependencies (shown in Table \ref{tab:Syntax}):
    
        \begin{table*}[!htb]
        \centering
        \caption{Overview of the information that is necessary to define each of the EDG elements.}
        \label{tab:Syntax}
        \resizebox{6.8in}{!}{%
            \begin{tabular}{@{}cll@{}}
                \toprule
                \multicolumn{1}{l}{SYMBOL}   & MEANING                                                                         & VALUES                                                                                      \\ \midrule
                $\rootnode$                  & \begin{tabular}[c]{@{}l@{}}Root Node /\\ Device Node\end{tabular}               & $\{ CPE_{current} \}$                                              \\
                                           &                                                                                 &                                                                                             \\
                $\assetnode$                 & Asset Node                                                                      & $\{ CPE_{previous}, CPE_{current}, CWE_{a_i}(t) \}$                                                  \\
                                           &                                                                                 &                                                                                             \\
                $\supernode$            & Supernode                                                                       & $\{ \{ CPE_{previous}, CPE_{current}, CWE_{a_i}(t) \}, \{ CVE_{a_i}(t), CVSS_{v_i}(t), CAPEC_{w_i}(t) \}, \{Dependencies\} \}$ \\
                                           &                                                                                 &                                                                                             \\
                $\vulnerabilitynode$       & Vulnerability Node                                                              & $\{ CVE, CVSS, CAPEC_{w_i}(t) \}$                                                              \\
                                           &                                                                                 &                                                                                             \\
                $\dependency$          & Dependency Relation                                                             &  ---                                                                                           \\
                                           &                                                                                 &                                                                                             \\
                $\update$          & \begin{tabular}[c]{@{}l@{}}Deprecated Asset /\\Deprecated Vulnerability\end{tabular} & ---                                                                                            \\ \bottomrule
            \end{tabular}%
        }
        \end{table*}
    
    
        \subsubsection{Root Node (RN)}
            Root nodes (collectively, set $G_{R}$) are represented within the graph as a square $\square$. Each node in this set represents the SUT. Each dependency tree will only have one single root node. The entire dependency tree starts from this node. Finally, each root node has a timestamp $(t)$ associated that indicates when the last check for updates was done. This timestamp is formatted following the structure defined in the ISO 8601 standard for date and time~\cite{ISO_2019_IDE}.
    
    
        \subsubsection{Asset Node (AN)}
            Asset nodes (collectively, set $G_{A}$) are represented within the graph as circles $\bigcirc$. Each node in this set represents an asset of the SUT. The EDG model does not impose any restrictions on the minimum number of assets the graph must have. However, the higher the number of assets, the better the SUT can be monitored over time. Moreover, the results and conclusions obtained will be much more accurate. That said, each EDG will have as many asset nodes as necessary, and the decomposition of assets can go as far and low-level as needed.
            
            Each known vulnerability node will be characterized by the following set of values:
    
            \begin{itemize}
                \item $CPE_{current}$: Current value for the CPE. It points to the current version of the asset it refers to.
                \item $CPE_{previous}$: Value of the CPE that identifies the previous version of this asset. It will be used by the model to trace back all the versions of the same asset in time, from the current one, to the very first one. 
                \item $CWE_{a_i}(t)$: Set of all weaknesses that are related to the vulnerabilities present in the asset. The content of this list can vary depending on the version of the asset.
            \end{itemize}
    
             Figure \ref{fig:cpe_relations}, illustrates an example of this approach. The solid line ($\longrightarrow$) of the arrow that points to $a_{i}$ indicates that the version $a_{i}$ is the current version of  asset $a$. The dotted arrows ($\dashrightarrow$) that point to $a_{2}$ and $a_{1}$ indicate that those are previous versions of  asset $a$. The last value of $CPE_{p_{1}}$  points to a null value, indicating that it is the last value, and therefore, the very first version of asset $a$.
    
            % =======
            % FIG. XX
            % =======
            \begin{figure}[!htb]
              \begin{center}
              \includegraphics[width=3.4in]{photo/cpe_relations.pdf}
              \caption{Tracking dependencies between the previous and current CPE values for asset $a$.}
              \label{fig:cpe_relations}
              \end{center}
            \end{figure}
    
    
        \subsubsection{Known Vulnerability Node (KVN)}
            Graphs alone cannot tell how severe or dangerous vulnerabilities might be. To develop structures that represent vulnerability relations, unique characterization of vulnerabilities is important~\cite{graphBasedSecurityIoT_2018}. Known vulnerability nodes (collectively, set $G_{V}$) are represented within the graph as black triangles $\blacktriangledown$. Each node in this set represents a known vulnerability present in the asset it relates to. Each asset will have a known vulnerability node for each known vulnerability belonging to that asset.
    
            To identify each known vulnerability node, each one will be characterized by the following set of features:
    
            \begin{itemize}
                \item $CVE$: This serves as the identifier of the vulnerability.
                \item $CVSS$: This metric assigns a numeric value to the severity of the vulnerability. Each CVE has a corresponding CVSS value.
                \item $\{ CAPEC \}$: Each vulnerability (CVE) is a materialization of a weakness (CWE) that can be exploited using a concrete attack pattern (CAPEC). In many cases, each CWE has more than one CAPEC associated, so this field is a set that contains all possible attack patterns that can exploit the vulnerability that is being analysed.
            \end{itemize}
    
    
        \subsubsection{Supernode (SN)}
        \label{subsec:supernode}
            Supernodes (collectively, set $G_{S}$) are represented within the graph as dotted circles $\dottedcircle$. Each node in this set represents a set of assets, their vulnerabilities, their dependencies, and their corresponding metrics (\textit{i.e.}, $CPE$, $CWE$, $CVE$, $CVSS$, and $CAPEC$). This special class of nodes will be used to further simplify the obtained graph, showing just the most relevant information in each case.
    
            To identify each supernode, and to be able to recover the information that they summarize, each one will be characterized by the metrics that define each one of the elements that they contain. That is, they must have all the information related to the assets and vulnerabilities that they summarize, along with their dependencies:
    
            \begin{itemize}
                \item $\{ CPE_{previous}, CPE_{current}, CWE_{a_i}(t) \}$: Identifiers for each asset to trace their versions until the very beginning.
                \item $\left( CVE, CVSS, \{ CAPEC \right) \}$: Identifiers for each vulnerability.
                \item $\{Dependencies\}$: It is an adjacency matrix that contains all relations among the elements inside the supernode structure.
            \end{itemize}
    
            Two types of criteria can be used to create supernodes and simplify the obtained graph:
            
            \begin{enumerate}
                \item \textbf{Presence of vulnerabilities}: Using this criterion, supernodes will group all nodes that contain no vulnerabilities associated. This can be seen in the lower side of Figure \ref{fig:supernode_CriteriaapplicationExamples}. In Figure \ref{fig:supernode_CriteriaapplicationExamples} b2), the nodes that can be grouped are detected, and finally, in Figure \ref{fig:supernode_CriteriaapplicationExamples} c2), they are substituted by their corresponding supernode.
    
                    % =======
                    % FIG. XX
                    % =======
                    \begin{figure*}[!htb]
                      \begin{center}
                      \includegraphics[width=6.8in]{photo/supernode.pdf}
                      \caption{Creating supernodes. Application of the two proposed criteria to the creation of supernodes to simplify the graph: 
                      (1) Establishing a threshold to select which vulnerability stays outside the supernode (upper side). 
                      (2) Choosing the presence of vulnerability as the criterion to create supernodes (lower side). The severity value (CVSS) for $v_{211}$ and $v_{212}$ is supposed to be lower than the establish threshold.}
                      \label{fig:supernode_CriteriaapplicationExamples}
                      \end{center}
                    \end{figure*}
    
                \item \textbf{CVSS Score below a certain threshold}: With this criterion, a threshold for the CVSS scores will be chosen. Every node that has no vulnerability will be simplified as in the previous case. In contrast, nodes whose CVSS score is less than the defined threshold will also be grouped into a supernode. This is illustrated in the upper side of Figure \ref{fig:supernode_CriteriaapplicationExamples}, in cases b1) and c1).
            \end{enumerate}
    
            It is worth noticing that applying the second set of criteria (establishing a CVSS threshold) will always return a graph that is at least as simple or as complex as the one that would be obtained using the presence of a vulnerability criterion. In the best case, the graph will be simpler. This is because both criteria treat assets with no vulnerabilities in the same way, so those will always be simplified. On the other hand, establishing a CVSS threshold allows the model for further simplifications.
            
            Moreover, the proposed model considers the time dimension (as will be explained in further sections), so all described criteria can also be applied over time. And if the information obtained over time is not of interest, it can be neglected, considering just the present time.
            
            On the other hand, all previously described criteria can be applied either globally, or locally to the area of the graph of interest of the analysis.
    
    
        \subsubsection{Normal dependency}
            This kind of dependency is represented within the graph as an arrow $\longrightarrow$ pointing from the source element ($S$) to the destination asset or vulnerability ($D$). This represents that the destination element depends on the source element. Collectively, these are known as set $G_D$.
    
    
        \subsubsection{Deprecated asset or vulnerability}
            This kind of dependency is represented within the graph as a dotted arrow $\dashrightarrow$ pointing from the source element ($S$) to the destination asset or vulnerability ($D$). This represents that the destination element used to depend on the source element. Collectively, these are known as set $G_U$.
    
            Having the possibility of representing old dependencies brings the opportunity to reflect graphically the evolution of the SUT over time. When a new version of an asset is released, or a vulnerability is patched (\textit{i.e.}, through an update), the model will be updated, and their dependencies will change from a normal dependency ($\longrightarrow$) to a deprecated asset or vulnerability dependency ($\dashrightarrow$) to reflect that change.
            
            
            
% @techreport{iso_central_secretary_systems_2016,
%   address = {Geneva, CH},
%   type = {Standard},
%   title = {Systems and software engineering -- {Lifecycle} profiles for {Very} {Small} {Entities} ({VSEs}) -- {Part} 1: {Overview}},
%   shorttitle = {{ISO}/{IEC} {TR} 29110-1:2016},
%   url = {https://www.iso.org/standard/62711.html},
%   language = {en},
%   number = {ISO/IEC TR 29110-1:2016},
%   institution = {International Organization for Standardization},
%   author = {{ISO Central Secretary}},
%   year = {2016}
% }

==> docs/discussion.tex <==
% =================================================================================
% === IX. Discussion ==============================================================
% =================================================================================
\section{Discussion}
\label{sec:discussion}
    % Quizás esto tiene que comentar la parte del caso de uso
    In the previous section, the EDG model and the proposed metrics were used to analyze the OpenPLC project throughout if whole life. The results of this vulnerability assessment have demonstrated the advantages and potential of our contribution.
    
    The first part of this analysis is the generation of the EDG for each version of OpenPLC. These graphs (Figure \ref{fig:openplcV1}, Figure \ref{fig:openplcV2}, and Figure \ref{fig:openplcV3}) serve as a visual tool for the evaluators, helping them to know the preliminary status of the SUT, before any further analysis. Taking an initial look at the EDG for OpenPLC V1, the dependency relation among the assets are easily identifiable. Furthermore, this dependency relation can help to examine which assets are affected by the exploitation of a certain vulnerability, and how it would propagate throughout the SUT.
    
    The remaining part of the analysis is the calculation of metrics. Continuing with OpenPLC V1, weaknesses found in the analysis can be classified into four main groups: 
    (1) Weaknesses related to buffer management operations, 
    (2) improper input validation,  
    (3) cryptographic issues, and 
    (4) resource management. 
    The CWE database itself provides a comprehensive list of requirements and tasks to perform during the development, test and maintenance phases. Using all this information, it is possible to:
    
    \begin{itemize}
        \item \textbf{Propose training:} The majority of the security issues of OpenPLC V1 come from the CWE-119 (15 out of 91 vulnerabilities) which is related to buffer overflow; and CWE-310 (12 out of 91 vulnerabilities) which is related to cryptographic issues. To prevent this from happening, training sessions for the developers can be organized to teach them how to avoid those problems.
        \item \textbf{Generate new requirements:} Sometimes it is enough to extract requirements from these CWE values, instead of proposing training. 
        \item \textbf{Generate new test cases:} In both cases (\textit{i.e.}, when proposing training or generating requirements), the corresponding tests can be generated from the corresponding CAPEC of each weakness. This will serve to further check whether the issue has been addressed.
    \end{itemize}
    
    

Two of them are related to the CWE-119\footnote{\href{https://cwe.mitre.org/data/definitions/119.html}{CWE-119}: ``The software performs operations on a memory buffer, but it can read from or write to a memory location that is outside the intended boundary of the buffer.''}.

elated to the CWE-426\footnote{\href{https://cwe.mitre.org/data/definitions/426.html}{CWE-426}: ``The application searches for critical resources using an externally-supplied search path that can point to resources that are not under the application's direct control.''}.

    All these results can be used to:

    \begin{itemize}
        \item \textbf{Tracking security issues:} Security vulnerabilities that are fixed should not appear in the next version of the EDG. So when they disappeared, the issue can be closed.
        \item \textbf{Penetration testing:} The number of vulnerabilities in the assets, the value of the CVSS for each one, and the CAPECs serve as an orientation for the pentester to choose a starting point.
        \item \textbf{Update management:} Severity values of CVSS, the existence of exploits, existing patches, and the number of vulnerabilities in each asset serve as a reference to decide whether to apply an update.
    \end{itemize}

    The analysis process described in this section can be further enhanced by extending the conclusions to the time dimension, instead of studying only OpenPLC V1. That is, drawing conclusions for all three versions of OpenPLC, from the obtained metrics.
    
    Finally, this approach is prone to automation, reducing the effort necessary to generate the model and update the data over time. Alerts and warnings can also be programmed in the case of excessively high CVSS values, or metrics outside established bounds. 
